Dual-Encoders for Extreme Multi-Label Classification

Dual-encoder (DE) models are widely used in retrieval tasks, most commonly studied on open QA benchmarks that are often characterized by multi-class and limited training data. In contrast, their performance in multi-label and data-rich retrieval settings like extreme multi-label classification (XMC), remains under-explored. Current empirical evidence indicates that DE models fall significantly short on XMC benchmarks, where SOTA methods linearly scale the number of learnable parameters with the total number of classes (documents in the corpus) by employing per-class classification head. To this end, we first study and highlight that existing multi-label contrastive training losses are not appropriate for training DE models on XMC tasks. We propose decoupled softmax loss - a simple modification to the InfoNCE loss - that overcomes the limitations of existing contrastive losses. We further extend our loss design to a soft top-k operator-based loss which is tailored to optimize top-k prediction performance. When trained with our proposed loss functions, standard DE models alone can match or outperform SOTA methods by up to 2% at Precision@1 even on the largest XMC datasets while being 20x smaller in terms of the number of trainable parameters. This leads to more parameter-efficient and universally applicable solutions for retrieval tasks. Our code and models are publicly available at https://github.com/nilesh2797/dexml.

==> new_introduction.tex <==
\section{Introduction}
\label{sec:intro}
Dual-encoder (DE) models have been highly successful in dense retrieval tasks for open-domain question answering (openQA) systems~\citep{Lee:2019, karpukhin2020dpr, qu2021rocketqa}, where they efficiently retrieve relevant passages or documents from a large corpus given a user's query. These models excel at leveraging their learned representations to identify and rank pertinent documents, by mapping both queries and documents into a shared embedding space, enabling efficient and effective retrieval using {\em fast similarity search methods}~\citep{Guo:2020ScaNN, Johnson:2021FAISS}. So far, DE models have been primarily explored in the zero-shot and the few-shot scenarios, where the models are required to {\em generalize} and retrieve relevant documents even though they might not have appeared in the training set.

An important retrieval scenario that frequently arises in real-world applications such as search engines~\citep{Mitra:2018Now} and recommendation systems~\citep{covington2016yt,Zhang:2019Survey} is where we want to perform retrieval for documents/items from a large collection based on a significant number of seen examples per document/item, i.e., a \textit{many-shot scenario}. Such tasks are often formulated as extreme multi-label classification (XMC) task, where each document/item to be retrieved is considered as a separate label~\citep{Bhatia16}. Typically, XMC algorithms need to both ``memorize'' and ``generalize''. That is, for each label they need to memorize the type of queries that are relevant; e.g., for a product to product recommendation scenario, the algorithm should memorize which products can lead to click on a particular product using the provided product-product co-click data. At the same time, the algorithm should generalize on unseen queries.

It is a prevailing belief in the XMC community that due to the semantic gap\todoasr{Should we say what `semantic gap` actually is?} and knowledge-intensive nature of XMC benchmarks, DE by themselves are not sufficient to attain good performance~\citep{dahiya23dexa}. As a measure to overcome the semantic gap and enable memorization, SOTA XMC methods augment DE with either per-label classifiers ~\citep{Dahiya23, mittal2021decaf} or extra auxiliary parameters~\citep{dahiya23dexa}. % to overcome the semantic gap and enable memorization. 
We explore this belief by performing a simple experiment on a synthetic dataset where a random query text is associated with a random document text, and the task is to memorize these random correlations during retrieval. As shown in Section ~\ref{app:synthetic_de_mem}, DE models are able to perform this task with perfect accuracy at least on up to 1M scale datasets, disputing the previously held belief in the literature.

\begin{wrapfigure}{r}{0.4\linewidth}
    \vspace{-12pt}
    \includegraphics[width=0.39\columnwidth]{images/params_vs_prec.pdf}
            \caption{\small Number of trainable parameters used by different models and their P@1 performance on LF-AmazonTitles-1.3M dataset}
    \label{fig:model_size}
    \vspace{-11pt}
\end{wrapfigure}
% \sout{In this work, we study this question}
In light of the aforementioned synthetic experiment, this work aims to answer the following question:
%
%\begin{center}
{``Are pure DE models sufficient for XMC tasks?''}
%\end{center}
Our findings reveal that DE models can match or even surpass state-of-the-art methods, achieving this feat without the need for per-label classifiers. This advancement bears significant implications:For XMC methods, unlike DE, the model size and consequently the number of trainable parameters scales {\em linearly} with the number of labels (see Figure~\ref{fig:model_size}).
%{\bf a.} For SOTA extreme classification methods, the classification network's size and consequently the number of trainable parameters scale {\em linearly} with the number of labels. That is, for say $1$B labels -- a reasonable setting for many web-scale systems -- model size would be about 256GB! In contrast, DE parameters tend to be independent of the number of labels -- assuming the encoder network size is kept fixed. See Figure~\ref{fig:model_size} for a comparison of a number of trainable parameters on different extreme classification benchmarks.
{2).} XMC methods require re-training or model updates on encountering new labels. In contrast, DE methods can generalize to new labels based on their features. 
Interestingly, our work shows that pure DE models can indeed match or even outperform SOTA XMC methods by up to 2\% even on the largest public XMC benchmarks while being 20$\times$ smaller in model size. The key to the improved performance is the right loss formulation for the underlying task and the use of extensive negatives to give consistent and unbiased loss feedback.

Our proposed changes to DE training are based on the observation that XMC problems involve multiple positives per query and a long tail of labels, which at query level manifests as a large number of highly relevant negatives.\todoasr{Elaborate?} Standard contrastive learning losses used to train DE models, e.g., InfoNCE loss~\citep{oord2018representation}, are not well-suited for multi-label learning tasks. Moreover, due to the computational requirements posed by encoding a large number of negative labels per query, standard approaches do not train DE models with sufficient number of negatives, whereas typical extreme classifiers are trained with significantly more ($\mathcal{O}(100)$) negatives per query. 
% For a batch size of 1K if we sample $\mathcal{O}(100)$ labels per sample then we would need to embed $\mathcal{O}(100K)$ labels per batch which is expensive and will lead to OOM with naive implementation.
We provide a simple fix to InfoNCE loss to allow for multi-label correlation between query and labels by proposing a decoupled loss that decomposes the loss over individual positives. This is required since standard contrastive losses forces all positive labels to have scores in similar range but not all positive labels possess equal ease of prediction from the available data. For example, in EURLex-4K dataset labels ``afghanistan'' and ``international\_sanctions'' often occur together but ``afghanistan'' is much easier to infer from the query text than ``international\_sanctions''. In Section ~\ref{sec:mthodology} we provide a more detailed motivation/justification for our proposed change to the InfoNCE loss. To establish the capabilities of DE methods, we first study our proposed loss using {\em all} the negatives in the loss term.  Naturally, including all negatives is challenging for million-label scale datasets. To this end, we provide a memory-efficient distributed implementation that %is able to 
can use multiple GPUs and a modified gradient cache~\citep{gao-etal-2021-scaling} approach to scale DE training to largest public XMC benchmarks even with a modest GPU setup (see Table~\ref{tab:main_results}, ~\ref{tab:runtimes}).
We further study the performances and implications of approximations of the proposed loss functions using standard hard negative mining approaches.
{Since many practical settings focus on \topk{} ranking performance, we further refine our loss design to this end. %We propose a loss function 
Based on a soft \textit{differentiable} version of \topk{} operation, we propose a novel loss function 
%\todoasr{@Nilesh: Can we call this loss function *novel*?}\todong{its semi-novel as I haven't seen this kind of formulation in literature for optimizing top-k, although our soft-topk operator is not novel} 
and show it can be integrated easily with standard DE training.
}

% \section{Old Introduction}
% \label{sec:old_intro}
% Dual-encoder (DE) models have been highly successful in dense retrieval tasks for open-domain question answering (openQA) systems~\citep{Lee:2019, karpukhin2020dpr, qu2021rocketqa}, where they efficiently retrieve relevant passages or documents from a large corpus given a user's query. These models excel at leveraging their learned representations to identify and rank pertinent documents, by mapping both queries and documents into a shared embedding space, enabling efficient and effective retrieval using {\em fast similarity search methods}~\citep{Guo:2020ScaNN, Johnson:2021FAISS}. So far, DE models have been primarily explored in the zero-shot and the few-shot scenarios, where the models are required to {\em generalize} and retrieve relevant documents even though they might not have appeared in the training set. %In these scenarios, DE models excel at leveraging their learned representations to identify and rank pertinent documents, playing a crucial role in the development of robust and accurate QA systems.

% Many-shot retrieval %scenarios are a
% is a distinct class of retrieval 
% tasks that involve learning to %classify or 
% retrieve relevant documents/items from a large collection based on a significant number of seen examples per document/item. Typically, these retrieval tasks can %also 
% be modeled as a multi-label classification problem, %where each %\sout{retrieval task}
% with each {candidate document}
% %\todong{task or document?} 
% % can be considered 
% representing as a separate label. These problems frequently emerge in real-world applications like search engines~\citep{Mitra:2018Now}, recommendation systems~\citep{covington2016yt,Zhang:2019Survey}, and document retrieval~\citep{macavaney2019cedr}, where the number of labels can easily run into millions or even billions~\citep{overwijk2022clueweb22} -- hence the name of extreme classification. For example, let us consider the problem of product-product recommendation -- similar to LF-AmazonTitles131K/1.3M datasets -- which can be modeled as many-shot retrieval or extreme multi-label classification. Given an input query, which is a product, the goal is to retrieve a ranked list of related products. % Generally, the catalog of products to be recommended does not change frequently, 
% Here, each product in the catalog can be considered as a separate {label}.
% %Here the goal is to retrieve a ranked list of related products for an input product. So the input query is a product and the item/document to be retrieved is also a product. Generally, the catalog of products to be recommended does not change often, so each product in the catalog can be considered as a separate {\em label}. %The number of labels can easily run into millions. 
% %

% Typically, the many-shot or multi-label algorithms need to both ``memorize'' and ``generalize''. That is, for each label they need to memorize the type of queries that are relevant; for example, memorize which products can lead to click on a particular product using the provided product-product co-click data. At the same time, the algorithm should generalize on unseen queries (new products in this case).
% %
% %Extreme classification benchmarks~\citep{Bhatia16}\todoasr{Are the additional repositories or benchmarks that we can cite?} are closely related to many-shot retrieval problems, as they require models to handle a massive number of classes or labels, often with thousands or millions of possible outcomes\todoasr{Not sure what ``outcome'' refers to here?}. These benchmarks serve as a testing ground for models, pushing their limits to effectively scale and handle the complexity of large-scale, many-shot retrieval scenarios.
% %
% \begin{wrapfigure}{r}{0.4\linewidth}
%     \vspace{-12pt}
%     \includegraphics[width=0.39\columnwidth]{images/model_size_comparison.pdf}
%             \caption{\small Number of trainable parameters used by DE models and SOTA extreme classification methods (NGAME and ELIAS) on different benchmarks~\citep{Bhatia16}.}
%     \label{fig:model_size}
%     \vspace{-11pt}
% \end{wrapfigure}
% State-of-the-art (SOTA) extreme classification methods exploit the above intuition by employing a hybrid approach of combining DE architectures with  {\em classification networks} --  a network with a separate classification head for each label. DE models' utilization of shared query and document embedding space helps them %map queries and items into a shared embedding space which helps to 
% generalize to new queries, while classification networks can leverage % models each label individually with 
% label-specific parameters to memorize relevant query features for each label. 
% %\todoasr{Maybe we can defined what exactly we mean by `classification networks`?} 
% %to address the challenges posed by extreme classification benchmarks~\citep{Dahiya23}. 
%  %DE models excel at mapping queries and items into a shared embedding space for efficient retrieval. However, they have been shown to underperform in extreme classification scenarios compared to the hybrid approach. The enhanced performance of the hybrid approach is attributed to the classification network's ability to model each label individually with label-specific classifier parameters. 
%  \iffalse
%  \sout{This can also potentially help in handling data where features are insufficient or misleading for explaining %\sout{data correlations}
% {\em the underlying query-document relevance}. }
% % \todong{maybe we should discuss other extreme classification approaches here, and highlight some of the differences between existing DE and extreme classification approaches}
% \fi
% On the other hand, training and maintaining such extreme classification techniques can be more challenging compared to the standard DE based approaches due to multiple reasons:\\
% {\bf a.} For extreme classification methods, unlike DE, the model size and consequently the number of trainable parameters scales {\em linearly} with the number of labels (see Figure~\ref{fig:model_size}). Here we are only comparing the trainable model parameters, DE methods do need to generate and store embeddings during inference using nearest-neighbor approaches. \\
% %{\bf a.} For SOTA extreme classification methods, the classification network's size and consequently the number of trainable parameters scale {\em linearly} with the number of labels. That is, for say $1$B labels -- a reasonable setting for many web-scale systems -- model size would be about 256GB! In contrast, DE parameters tend to be independent of the number of labels -- assuming the encoder network size is kept fixed. See Figure~\ref{fig:model_size} for a comparison of a number of trainable parameters on different extreme classification benchmarks.
% {\bf b.} Extreme classification methods require re-training or model updates on encountering new labels. In contrast, DE methods can generalize to new labels based on their features. \\
% %{\bf b.} In practice, we might encounter new labels fairly often, e.g., product catalog can be updated for retailers almost every week. This requires model re-training or at least model updates in extreme classification methods. In contrast, DE methods can generalize to new labels based on their features.  \\ %Such requirement is not there for the DE techniques.\\
% {\bf c.} Vanilla extreme classification methods ignore label similarity while treating two similar products as separate labels, leading to potential uneven performance for such products. DE embed similar products closely by leveraging their common features and joint data, leading to a similar performance.
% %{\bf c.} Many times certain labels might be very similar, e.g. two products with almost the same title. Vanilla extreme classification methods would still treat them separately, and hence one label might have a lot of positive query data but the other close label might be data starved, leading to uneven performance. For DE, generally such cases would lead to closely embedded labels and smooth classification function in the embedding space which allows for sharing of data. 

% Despite the above advantages of DE models, extreme classification techniques are still widely applied in many-shot retrieval applications perhaps due to their superior performance. We are able to validate this hypothesis on a variety of extreme classification benchmarks; see Table~\ref{tab:main_results}. For example, on LF-AmazonTitles-1.3M dataset, standard DE based approaches under-perform by as much as 7.5\%, in Precision@1, than the SOTA extreme classification techniques with exactly the {\em same} query encoder architecture. %\sout{A natural suspicion for this observation is that extreme classification methods due to a large number of trainable parameters have a significant advantage over pure DE based approaches, as they can model individual labels separately instead of fitting all of them in the same embedding space.}
% {It is natural to suspect that the seemingly limited capacity of DE models due to their fixed size is the reason behind this quality gap.} %\todo{same embedding space or modeled by the same limited shared parameters?}

% In this paper, we investigate if this is indeed the case %\sout{-- at least for practical extreme classification benchmarks --} 
% or whether the standard training of DE methods is not suitable for many-shot retrieval based multi-label tasks. %In this paper, we 
% Our exploration validates the latter hypothesis. Indeed, we could modify the DE training procedure % we are able to change the loss function and hence the training procedure of DE methods 
% to match and in some cases, even surpass the performance of multi-label specific extreme classification techniques. For example, on the AmazonTitles-1.3M dataset mentioned above, our modified DE training leads to an improvement of 9\% in Precision@1, thus surpassing the SOTA extreme classification results by about~1.6\%. 

% Our proposed changes to DE training are based on the observation that extreme classification problems can involve a long tail of labels, which at query level manifests as multiple positives and a large number of highly relevant negatives. Standard contrastive learning losses used to train DE, e.g., InfoNCE loss~\citep{oord2018representation}, are not well-suited for multiple positive labels associated with a query. % as well as can lead to high bias or variance in the estimation of loss term corresponding to negative labels for a given query. 
% Moreover, the bias or variance introduced by \textit{negative sampling} %towards estimating the underlying full loss 
% also degrades the quality of the resulting 
% DE model. We provide a simple fix by proposing a decoupled loss that decomposes the loss over all positives, and use {\em all} the negatives in the loss term, thus completely removing the bias/variance challenge. Naturally, including all negatives is challenging for million-label scale datasets. To this end, we provide a memory-efficient distributed implementation that %is able to 
% can use multiple GPUs to scale the method to million-scale %, so that the hypothesis can be proven for such datasets 
% (see Table~\ref{tab:main_results}). {Since many practical settings focus on \topk{} ranking performance, we further refine our loss design to this end. %We propose a loss function 
% Based on a soft \textit{differentiable} version of \topk{} operation, we propose a novel loss function 
% %\todoasr{@Nilesh: Can we call this loss function *novel*?}\todong{its semi-novel as I haven't seen this kind of formulation in literature for optimizing top-k, although our soft-topk operator is not novel} 
% and show it can be integrated easily with standard DE training.
% }
% %We further refine the loss function to focus on top-K retrieved labels, as most such problems are used in topK kind of ranking scenarios. We proposed a soft-topK operator based loss function, and show it can be integrated easily with standard DE training. 
% Our experiments on extreme classification benchmarks indicate that \topk~based optimization can further improve %DE's 
% Precision@k by up to $1\%$ and Recall@k by up to $2\%$.  Finally, we investigate the effect of our DE training modifications % on multiple axes, including their impact 
% on head vs tail labels -- labels with many and very few query points in training set, respectively. 
% %In this paper, we investigate the efficacy of pure DE-based approaches for the extreme classification tasks, focusing on their potential to perform competitively without relying on additional classification networks. A pure DE approach can be preferred over a hybrid approach due to its simplified architecture and better generalization, and adaptability\todoasr{Maybe add `adaptability to what`?}. These characteristics make it a promising alternative for large-scale problems, particularly in scenarios where incorporating new classes or adjusting to evolving data is crucial. Our findings reveal that when DE models are trained with a large pool of negative examples, their performance can meet or even surpass SOTA extreme classification approaches. 
% In summary, our key contributions are as follows:
% \begin{itemize}[leftmargin=*]
%     \item  We investigate the efficacy of DE methods for many-shot retrieval %aka extreme multi-label classification, 
%     and empirically validate that existing DE methods  can be up to $7.5$\% less accurate than SOTA extreme classification methods. 
%     %that standard dual encoders' performance 
% %    in comparison to SOTA extreme %multi-label 
%  %   classification techniques. 
%     \item We \textit{invalidate} that it is the smaller model size that leads to under-performance. Instead, we identify that the current DE training strategy is one of the key reasons and propose simple yet effective multi-label specific modifications to the training objective that can boost the performance to surpass extreme classificaton methods by up to $2\%$ in terms of Precision@1 despite being $20\times$ smaller in number of parameters; see Table~\ref{tab:main_results}. 
%     %\todong{We propose simple yet effective modifications to existing DE training formulations to adapt for multi-label many-shot nature of extreme classification benchmarks leading to up to $2\%$ improvements at Precision@1 over SOTA methods while being $20\times$ smaller in number of parameters}
%     \item We further enhance DE training by using a soft \topk{} operator based loss function which allows DE to focus %training on just 
%     on getting the correct labels in \topk{} prediction slots as per the underlying metrics of interest. This can further improve the Recall@k and Precision@k up to $2\%$ and $1\%$, respectively
% \end{itemize}
% \vspace{-2mm}
% % 
% % \todoasr{Add a few sentences on the organization of the rest of the paper.}
Before providing a detailed account of our contributions in Section~\ref{sec:mthodology} and \ref{sec:experiments}, we begin by discussing relevant literature in Section~\ref{sec:related} and introducing necessary background in Section~\ref{sec:bg}.

==> results_and_discussion.tex <==
\section{Results and Discussion}
\begin{itemize}
    \item Comparison of enhanced two-tower models with one-tower models and existing two-tower models
    \item Insights into the performance gains
    \item Generalizability to other many-shot retrieval tasks
\end{itemize}

==> tables/full_our_results.tex <==
\setlength{\textfloatsep}{2pt}
\begin{table*}[!t]
    \caption{\small Full our results}
    \label{tab:full_our_results}
      \centering
      \resizebox{\linewidth}{!}{
        \begin{tabular}{@{}l|ccc|ccc|ccc|cccc@{}}
        \toprule
        \textbf{Method} & \textbf{P@1} & \textbf{P@3} & \textbf{P@5} & \textbf{N@1} & \textbf{N@3} & \textbf{N@5} & \textbf{PSP@1} & \textbf{PSP@3} & \textbf{PSP@5} & \textbf{R@10} & \textbf{R@20} & & \textbf{R@50} &\textbf{R@100}\\ \midrule
        
        & \multicolumn{12}{c}{EURLex-4K}\\ \midrule
        \midrule
        DistilBERT OvA Classifier & - & - & - & - & - & - & - & - & - & - & - & - & - \\
        In-batch DE & 83.98	& 69.34	& 56.29	& 83.98	& 73.23	& 66.47	& 41.82	& 48.88	& 51.48	& 67.51	& 75.91	& 83.68	& 88.22 \\
        Hard negative DE & 84.61	& 71.82	& 59.15	& 84.61	& 75.25	& 69	& 41.16	& 49.89	& 53.11	& 71.08	& 79.18	& 86.27	& 90.21 \\
        \dsloss~DE & 86.78	& 73.4	& 60.19	& 86.78	& 76.95	& 70.37	& 46.17	& 52.62	& 54.78	& 72.56	& 80.69	& 87.96	& 91.75 \\
        \stopat-$5$ DE & 83.42	& 72.03	& 60.95	& 83.42	& 75.15	& 70.07	& 45.68	& 52.9	& 56.84	& 74.21	& 81.85	& 88.14	& 91.3 \\
        \midrule
        & \multicolumn{12}{c}{LF-AmazonTitles-131K}\\ \midrule
        \midrule
        DistilBERT OvA Classifier \\
        In-batch DE \\
        Hard negative DE \\
        \dsloss~DE \\
        \stopat-$5$ DE \\
        \midrule
        & \multicolumn{12}{c}{LF-Wikipedia-500K}\\ \midrule
        \midrule
        DistilBERT OvA Classifier \\
        In-batch DE \\
        Hard negative DE \\
        \dsloss~DE \\
        \stopat-$5$ DE \\
        \midrule
        & \multicolumn{12}{c}{LF-AmazonTitles-1.3M}\\ \midrule
        \midrule
        DistilBERT OvA Classifier & 48.72 & 42.91 & 39.09 & 48.72 & 46 & 44.79 & 18.6 & 23.02 & 25.91 & 29.15 & 38.98 & 51.31 & 58.34 \\
        In-batch DE  & 42.15 & 36.84 & 32.97 & 42.15 & 40.7 & 39.86 & 29.37 & 31.78 & 33.08 & 29.28 & 38.27 & 50.19 & 57.48 \\
        Hard negative DE  & 49.16 & 43.39 & 39.07 & 49.16 & 47.62 & 46.64 & 29.26 & 32.29 & 34.02 & 32.76 & 42.06 & 53.55 & 60.09 \\
        \dsloss~DE \\
        \stopat-$5$ DE \\
        \bottomrule
    \end{tabular}}
\end{table*}

